Quasi-steady-state approximations derived from the stochastic model of enzyme kinetics

In this paper we derive several quasi steady-state approximations (QSSAs) to the stochastic reaction network describing the Michaelis-Menten enzyme kinetics. We show how the different assumptions about chemical species abundance and reaction rates lead to the standard QSSA (sQSSA), the total QSSA (tQSSA), and the reverse QSSA (rQSSA) approximations. These three QSSAs have been widely studied in the literature in deterministic ordinary differential equation (ODE) settings and several sets of conditions for their validity have been proposed. By using multiscaling techniques introduced in Kang (and Kurtz 2013) and Ball et al. (2006) we show that these conditions for deterministic QSSAs largely agree with the ones for QSSAs in the large volume limits of the underlying stochastic enzyme kinetic network.

==> Sections_v3/abstract.tex <==
\begin{abstract}
In this paper we derive several quasi steady-state approximations (QSSAs) to  the stochastic reaction network describing  the Michaelis-Menten enzyme kinetics. We show how   the different assumptions about chemical species abundance and reaction rates lead to the standard QSSA (sQSSA), the total QSSA (tQSSA), and the reverse QSSA (rQSSA) approximations. These three QSSAs have  been widely studied in the literature in deterministic ordinary differential equation (ODE)  settings  and several sets of conditions for their validity have been proposed.  By using multiscaling techniques  introduced in  \cite{Kang:2013:STM,Ball:2006:AAM} we   show that  these  conditions  for deterministic QSSAs largely agree with the ones  for  QSSAs  in   the large volume limits of the underlying stochastic enzyme kinetic network. 

\keywords{Michaelis-Menten kinetics \and Stochastic reaction network \and Multiscale approximation \and QSSA}
\subclass{60J27 \and 60J28 \and 34E15 \and 92C42 \and 92B25 \and 92C45}
\end{abstract}

